Generating Furry Cars: Disentangling Object Shape & Appearance across Multiple Domains

We consider the novel task of learning disentangled representations of object shape and appearance across multiple domains (e.g., dogs and cars). The goal is to learn a generative model that learns an intermediate distribution, which borrows a subset of properties from each domain, enabling the generation of images that did not exist in any domain exclusively. This challenging problem requires an accurate disentanglement of object shape, appearance, and background from each domain, so that the appearance and shape factors from the two domains can be interchanged. We augment an existing approach that can disentangle factors within a single domain but struggles to do so across domains. Our key technical contribution is to represent object appearance with a differentiable histogram of visual features, and to optimize the generator so that two images with the same latent appearance factor but different latent shape factors produce similar histograms. On multiple multi-domain datasets, we demonstrate our method leads to accurate and consistent appearance and shape transfer across domains.

==> approachv1.tex <==
\section{Approach}
Our goal is to jointly model a pair of image domains $\mathcal{A}$ and $\mathcal{B}$ in an unsupervised way, such that the resulting generative model can combine one latent factor from $\mathcal{A}$, another factor from $\mathcal{B}$,  to generate an image preserving the respective latent properties. 
%Fig.\ref{fig:hist} illustrates what constitutes an accurate combination, when the latent factors are shape and appearance. The toy example demonstrates three scenarios of combining the appearance of a rectangle-shaped object $O_1$ with the shapes of ellipse-shaped objects $O_2$, $O_3$ and $O_4$. The appearance to be transferred consists of two distinct features; a checkered and a plain blue pattern. Of the two, $O_3$ and $O_4$ represent what we consider a successful transfer in the context of this work. This is because the relative frequencies of the mentioned appearance features remain consistent in $O_3$, $O_4$ compared to $O_1$, which is not the case with $O_2$. Note that an object's size does not impact its normalized feature histogram. Also note that while transferring appearance to an arbitrary shape, there might no longer be any part correspondence (e.g. it is not clear where the appearance of a bird's head should get transferred to in a car). It is for that reason that we consider the case of $O_4$ as success, even if the relative positioning of features have changed.    
%Our idea borrows motivation through this analysis, where we seek to 
Focusing on object shape and appearance as latent factors in this work, our idea is to approximate feature histograms in a differentiable way. Doing so enables us to optimize our model, which is a deep neural network, in a way that constrains any two images having the same latent appearance to have similar feature histograms, thus helping the model learn a much better disentangled representations of mentioned factors. 
%Given a method which already performs well in terms of intra-domain disentanglement, our proposed framework intends to extend the method's ability from performing intra to inter-domain disentanglement. 

% In the remainder of this section, we first formalize the requirements needed off the method that is able to perform intra-domain disentanglement. We then explain our proposed framework, which includes approximating feature histograms in a differentiable way, and the corresponding loss functions. We finally explain how our framework can blend in with the method to help achieve inter-domain disentanglement. 
In the remainder of this section, we first formalize the properties that we desire out of our final model. We then discuss a subset of properties one can obtain through one of the existing intra-domain disentanglement works \citep{singh-cvpr2019}. Finally, we explain how our proposed framework can help develop a model which has the complete set of properties.
%can blend in with the existing work to help achieve the final set of properties.

\subsection{Problem formulation}\label{sec:formulation}
Combining factors from multiple domains, as illustrated in Fig.\ref{fig:teaser}, requires learning a disentangled latent representation for - (i) \emph{appearance of the foreground object}: this is because imagining the brown car in the red/blue bird's texture only alters the appearance of the car, and not its shape, background or pose ($I_3$ and $I_{AB}$); (ii) \emph{shape of the foreground object}: with similar reasoning, we need some way to ensure that the hybrid car ($I_{AB}$) has the same shape as the brown car; (iii) \emph{background}: this is because we desire the background to remain consistent when altering the foreground object properties (e.g. $I_1 \rightarrow I_{AA}$; $I_3 \rightarrow I_{BB}$). All the other continuous variations (e.g. pose, viewpoint of the foreground) can be represented through a noise vector. 

%So, the generative model $G$ should take four latent vectors as input for controlling the appearance, shape, pose and background of the object respectively. 
In this work, we specifically focus on shape and appearance (color and texture) as latent factors to be combined from different domains. As shown in Fig.\ref{fig:teaser}, we can interpret domain $\mathcal{A}$ as having an associated set of shapes - $X_{\mathcal{A}}$ (e.g. possible bird shapes), and an associated set of appearances - $Y_{\mathcal{A}}$ (e.g. possible bird appearances). With a similar interpretation for domain $\mathcal{B}$, we can formalize the following problems:

\textbf{Intra-domain disentanglement:} in this setup, we're only concerned if the method can generate images of the form $I = G(x, y, z, b)$, where $z, b$ control object pose and background respectively, and $[x,y] \in (X_A \times Y_A)$ ($\times$ denotes Cartesian product). In other words, the task is to combine all possible shapes with the possible appearances within a domain (e.g. $I_{AA}$ and $I_{BB}$ in Fig.\ref{fig:teaser}).\\ \textbf{Inter-domain disentanglement:} everything remains the same as intra-domain disentanglement, except that $[x,y] \in (X_{AB} \times Y_{AB})$, where $X_{AB} = (X_A \cup X_B)$ and $Y_{AB} = (Y_A \cup Y_B)$. This is a more general version of the previous task, where we wish to combine all possible shapes with all possible appearances across multiple domains (e.g. $I_{AB}$ in Fig.\ref{fig:teaser}).

% THIS IS ONE OF THE OPTIONS TO TALK ABOUT FINEGAN - To the best of our knowledge, FineGAN is the only existing work which can disentangle foreground, background etc.
We start with a \emph{base model} which can perform unsupervised intra-domain disentanglement \citep{singh-cvpr2019}, the properties of which are summarized in Fig.\ref{fig:base}. Specifically, the base model should take four latent vectors as input ($z$, $x$, $y$ and $b$), and generate an image whose object's appearance, shape, pose and background are controlled by each of the latent vectors independently. Note that disentangling the foreground from background requires the model to generate them separately, and combine them using a foreground mask to generate the final image : $I = (m*I_f) + (1-m)*I_b$, where $I_f$, $I_b$ and $m$ are foreground, background and mask respectively.   
We  now present our contributions which extend the method’s ability from performing intra to inter-domain disentanglement.
% In the context of this work, we say that a generative model $G_{\mathcal{A}}$ is able to perform intra-domain disentanglement on domain $\mathcal{A}$ (e.g. birds), if and only if it is able to disentangle four factors of variations - pose, shape, appearance and background - while generating an image. This means that $G_{\mathcal{A}}$ takes four latent variables as input (one for each factor), and each variable controls the corresponding factor in the generated image. Fig.\ref{fig:base} summarizes these properties of $G_{\mathcal{A}}$; in each row, only one factor varies left to right, and all the other factors remain the same. Note that in order to accurately disentangle background from foreground (last row in Fig.\ref{fig:base}), the model needs to generate foreground in a separate layer, and will consequently generate the corresponding mask to stitch it with the background [issues in describing the concept of mask without describing FineGAN].  
\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figs/base_model.pdf}
    \caption{Base model \citep{singh-cvpr2019} capable of performing intra-domain disentanglement for four factors of variation. Each of the four rows demonstrates the effect of changing one latent factor, which controls a single attribute in the image.}
    \label{fig:base}
\end{figure}

\subsection{Differentiable approximation of feature histograms}\label{sec:approx}
%The same base model which can combine shape and appearance effectively within a domain has trouble combining them across different ones. 
Although the base model can combine shape and appearance effectively within a single domain (Fig. \ref{fig:base} bottom left), it has trouble doing so across different ones. This is illustrated in Fig.\ref{fig:pos_neg}, where transferring the latent appearance of a car ($I$) to a bird's shape results in a foreground with entirely different appearance ($I_{pos_{2}}$ vs $I$), indicating an inconsistent behavior across different domains. In this context, a natural way to think of a \emph{consistent} behavior is when the frequency of most visual features (e.g. RGB color distribution) remain similar when an appearance is combined with an arbitrary shape. Our idea hence revolves around constructing frequency based representations of foreground appearance, which needs to follow two properties - (i) representations should be able to capture the frequency of arbitrary visual features (e.g. red color, dog's fur, leopard's texture); (ii) construction process should be differentiable, so as to incorporate histogram equalization (e.g. of $I$ and $I_{pos_{2}}$) as part of the optimization process.   
%Ideally, we would want a bird whose body is mostly red, and partially blue (taken from the car's window panes).   
%The objective is for any two images $I_1 = G(x_1, y, z_1, b_1)$ and $I_2 = G(x_2, y, z_2, b_2)$ (having same latent representation for appearance, $y$) to have similar feature histograms. Traditionally, methods like color histogram and textons [cite works] have been used to represent appearance properties such as relative frequencies of different colors and textures respectively. The reasons for them not being usable and suitable in this work's optimization setup is two-fold : (i) both algorithms employ hard assignment of each pixel to one of the clusters, which introduces non-differentiability; (ii) neither of them describe appearance holistically, as appearance in itself is a property which is a complex combination of color and texture.

 The construction of feature histograms is illustrated in Fig.\ref{fig:hist_rep}. We convolve a generated image $I$ (from base model) with a randomly initialized filter banks to get $k$ response maps. Our goal is to only consider the foreground during histogram approximation. Hence, we use the generated foreground mask $M$ of the image, and multiply element-wise with all the response maps. Finally, we compute channel-wise sum, and normalize it by \codeword{sum}$(M)$ to get the final $k$-dimensional histogram representation. For simplicity, we've only shown this process with one layer of filter bank; but note that one can further convolve the intermediate response map with another layer of filter bank, and repeat the same process to get the histogram representation at another level. In essence, we're finding regions in $I$ of high correlation with each filter $f_i$ in the bank. Summing up these correlations over the foreground body will hence indicate the frequency of the visual pattern represented by $f_i$. Note how this method results in soft assignment of each pixel value to one of the $k$ feature bins, and hence making it differentiable.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/hist_representation_new.pdf}
    \caption{Feature histogram approximation method. The base model, conditioned on multiple latent vectors, generates an image and it's foreground mask. Note that all the subsequent operations (e.g. convolution, element-wise multiplication) are differentiable, making the whole process usable for histogram equalization constraints.}
    \label{fig:hist_rep}
\end{figure}

Ideally, the patterns represented/captured by the filter bank should encompass all the low-level features present in the dataset (e.g. dog's fur, leopard's texture). This would make the histogram comparison most informative, as only the frequencies of \emph{relevant features} are used for comparison. In practice, however, designing such filter bank is intractable. We approximate the filter bank capturing the \emph{relevant features}, by adopting the following principle from contrastive learning literature \citep{bachman-neurips2019, chen-arxiv2020}; images \emph{known} to have same appearance should have similar feature histograms (positive examples), and the ones \emph{known} to have different appearance should have different feature histograms (negative examples). We first construct a batch of $N$ generated images, where each image is of the form $I = G(x_1, y_1, z_1, b_1)$. We then construct another batch, where each image is of the form $I_{pos_{1}} = G(x_1, y_1, z_2, b_1)$ by only altering the noise ($z$) vector. Note that it is the property of our \emph{base model} through which we can assume that changing the noise vector will accurately retain the appearance of the foreground object (first row of Fig.\ref{fig:base}). This way, each of the corresponding images in $I$ and $I_{pos_{1}}$ will be positive samples. We get the histogram representation for all the $2N$ images, and calculate the $NT$-$Xent$ (Normalized temperature-scaled cross entropy loss) for each image in the batch :

\begin{equation}
\ell_{i}=-\log \frac{\exp \left(\operatorname{sim}\left(h_{i}, h_{j}\right) / \tau\right)}{\sum_{k=1}^{2 N} \mathbf{1}_{[k \neq i]} \exp \left(\operatorname{sim}\left(h_{i}, h_{k}\right) / \tau\right)}
\label{eq:filter}
\end{equation}
where $h_{i}$ represents the feature histogram of $i^{th}$ image, $j$ indexes the positive sample for $i$, and $\tau$ represents the temperature hyperparameter.
%Note that the loss term mentioned in Eq.\ref{eq:filter} is computed for each image in $\mathcal{I}$.
We refer to the whole loss as $L_{filter} = \sum_{i=1}^{N} \ell_{i}$, and optimize it by only updating the weights of the filter bank.

We now define the objective function for the core task our framework strives to solve - two images having different shapes but same latent appearance representation should have similar feature histograms. For this, we again use $L_{filter}$ defined above, and use the same $I = G(x_1, y_1, z_1, b_1)$. We construct the positive samples, however, differently - $I_{pos_{2}} = G(x_2, y_1, z_1, b_1)$ (latent shape representation $x$ is different). We refer to this loss as $L_{hist}$, and optimize $G$'s parameters, while keeping the weights of the filter banks fixed. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/contrastive_new.pdf}
    \caption{Positive/negative samples for different loss functions. Positive samples for $L_{filter}$ are the ones that we \emph{know} have similar appearance, whereas the positive samples for $L_{hist}$ are the ones that we \emph{wish} to have similar appearance. Negative samples remain the same for both $L_{filter}$ and $L_{hist}$.}
    \label{fig:pos_neg}
\end{figure}

% \begin{figure}
%     \centering
%     \subfloat[]{{\includegraphics[width=0.31\textwidth]{figs/diff_transfers.pdf}}}
%     \qquad
%     \subfloat[]{{\includegraphics[width=0.62\textwidth]{figs/contrastive_new.pdf}}}
%     \caption{(a) Transferring a car's appearance to a bird's body; (b) Positive/negative samples for different loss functions}
%     \label{fig:pos_neg}
% \end{figure}


Fig.\ref{fig:pos_neg} summarizes the idea of positive and negative samples for $L_{filter}$ and $L_{hist}$. On a high level, $L_{hist}$ ensures that the latent appearance's behavior is shape/domain invariant, i.e. like a blanket of appearance details which can be wrapped around any object shape. 

\subsection{Base model}\label{sec:base_sec}
In principle, the framework described above should work with any base model that has the properties required to perform intra-domain disentanglement, as decsribed in Sec. \ref{sec:formulation}. To the best of our knowledge, however, FineGAN \citep{singh-cvpr2019} is the only method meeting those requirements in an unsupervised manner. 
%To the best of our knowledge, however, the only method capable of performing intra-domain disentanglement is FineGAN \cite{singh-cvpr2019}. 
It takes in four latent variables as input - a continuous noise vector $z \sim \mathcal{N}(0,1)$, and one-hot vectors $x \sim \text{Cat}(K = N_x,p = 1/N_x)$, $y \sim \text{Cat}(K = N_y,p = 1/N_y)$ and $b \sim \text{Cat}(K = N_b,p = 1/N_b)$, where $N_x$, $N_y$ and $N_b$ represent the number of distinct shapes, appearances and background of objects in a dataset. FineGAN takes in these sampled codes, and generates an image in a stagewise manner, where $b$ first generates a realistic background, ${x,z}$ synthesizes the silhouette (shape) of the foreground object, and $y$ fills in the appearance details in the silhouette. To generate the final image $I$ combining all these different parts, the model also generates a foreground mask  $m$ in an \emph{unsupervised} way, and uses it to stitch the foreground and background. To learn the desired disentanglement, FineGAN makes the assumption that $N_x < N_y$, i.e. varieties in shapes is less than different appearances of objects. This is especially true in the context of fine-grained image datasets, for e.g. all ducks having different appearances have the same overall shape. During training, this \emph{hierarchy constraint} is imposed in the process of constructing latent vectors, where a set of appearance vectors ($y$) will always be paired with a particular shape vector ($x$). This ensures that, during training, the shape vector representing the duck's shape does not get paired up with the appearance vector for sparrow's texture to create some unnatural combination (which could be used by a discriminator to easily classify the image as fake). Two types of loss functions are used - $L_{abv}$, i.e. the adversarial losses \citep{goodfellow-nips2014} to enforce realism on the background image and the final image ($I$), and mutual information loss $L_{info}$ \citep{chen-nips16} between (i) $x$ and foreground shape, (ii) $y$ and foreground appearance, to help the latent vectors get control over the respective factors. We denote the loss functions used by the base model (FineGAN in this case) as $L_{base}$.
%and generates an image in a stagewise manner where the appearance, shape, pose and background of the object can be controlled independently (Fig.~\ref{fig:base}). The core idea is centered around an observation that if two object categories are similar in shape but have differing appearance (e.g. two different duck species), then this could be understood as similarity in one of the latent factors, and difference in some other. Consequently, a hierarchy of latent factors could be imagined, where a set of object categories would have the same parent latent factor (e.g. common shape). To model this, FineGAN constructs its latent space in a hierarchical manner, where a set of $y$ (appearance codes) are constrained to have same $x$ (shape code) during training. The overall generation process is broken down into multiple stages, where each subsequent stage adds more details to the image. First, a background stage (conditioned on $b$ and $z$) generates a realistic background. 
%by modeling it on a patch level, i.e. real images are patches outside the bounding box in real images. 
%The parent stage (conditioned on $x$ and $z$) then synthesizes the silhouette (shape) of the final object to be generated, and also generates a mask to combine it with the background image. Finally, the child stage (conditioned on $y$) fills in the appearance details to complete the generation process. The background and child stage uses standard adversarial losses to enforce realism in background and final images respectively, and the parent and child stage maximize the mutual information between the latent codes ($x$ and $y$) and their respective images, so as to enable the latent vectors gain control over the respective properties. 
So, the overall loss function used by our framework becomes:
\begin{equation}
\mathcal{L} = L_{base} + L_{hist} + L_{filter}    
\end{equation}
where $L_{base}$ constrains the model to have the properties needed for intra-domain disentanglement, $L_{hist}$ constrains images having same latent appearance factor to have similar histogram, and $L_{filter}$ ensures that the filter bank used to approximate the histograms captures discriminative properties of the dataset.  
% If we wish for any two generated images $I_1$ and $I_2$ with arbitrary shapes to have the same appearance details, the idea of feature histogram equalization of $I_1$ and $I_2$ seems promising. But to ensure that background details are not considered as part of histogram equalization, our generative model needs to be able to disentangle background from foreground while generating the complete image. 
% To this end, we build upon the recent work of FineGAN [refer], which is an unsupervised generative model that can (i) disentangle the background from foreground; (ii) perform intra-domain disentanglement between shape and appearance, as described in Fig.\ref{fig:teaser}. In the next section, we briefly describe the core components of FineGAN, and give a high-level overview of it's strengths and weaknesses in terms of qualitative results. We then introduce our framework which can blend in with FineGAN's model to enable inter-domain disentanglement.

% \subsection{FineGAN}
% FineGAN proposed a generative model which can take in four latent variables $z$, $b$, $p$ and $c$
% The premise of FineGAN is centered around a property that many \emph{fine-grained} image datasets tend to follow: if the visual differences between images belonging to object category $c_1$ and $c_2$ are indeed fine-grained (e.g. only the spots on the tail of a bird are differently colored for $c_2$ than $c_1$, but the rest of the body is same as $c_1$), then this could be understood as similarity in one of the latent factors, and difference in some other. So, in a dataset of $n$ fine-grained categories, a hierarchy of latent factors could be imagined, where a subset of $n_1$ fine-grained categories would have the same parent latent factor $p_1$.

% The core idea of the work then becomes to disentangle the factors present at different levels of this potential hierarchy. Since there is no human-level annotation for this latent hierarchy, FineGAN assumes one based on some heuristics (e..g # of parent nodes < # of child nodes; some children will share the same parent nodes). This hierarchy is enforced through the latent variables  


==> approachv2.tex <==
\section{Approach}
Our goal is to jointly model a pair of image domains $\mathcal{A}$ and $\mathcal{B}$ in an unsupervised way, such that the resulting generative model can combine one latent factor from $\mathcal{A}$, another factor from $\mathcal{B}$,  to generate an out-of-distribution image preserving the latent properties from respective distributions. 
Focusing on object shape and appearance as latent factors in this work, our idea is to capture the appearance through feature histograms in a differentiable way. Doing so enables us to optimize our model, which is a deep neural network, in a way that constrains any two images having the same latent appearance to have similar feature histograms, thus similar appearance. Consequently, the model learns a much better disentangled representations of mentioned factors across multiple domains. 

In the remainder of this section, we first formalize the properties that we desire out of our final model. We then discuss a subset of properties one can obtain through one of the existing works \citep{singh-cvpr2019}. Finally, we explain how our proposed framework can help develop a model which has the complete set of properties.
%can blend in with the existing work to help achieve the final set of properties.

\subsection{Problem formulation}\label{sec:formulation}
Combining factors from multiple domains, as illustrated in Fig.\ref{fig:teaser}, requires learning a disentangled latent representation for \emph{appearance, shape and background} of an object. This enables each of the latent factors' behavior to remain consistent, irrespective of the other factors. For example, the latent vector for red/blue color results in same appearance when combined with a bird's shape ($I_{AA}$ in Fig.\ref{fig:teaser}) or a car's shape ($I_{AB}$). Henceforth, we will represent shape, appearance and background of an object as $x$, $y$, $b$ respectively, and remaining continuous factors (e.g. object pose) using $z$.

As shown in Fig.\ref{fig:teaser}, we can interpret domain $\mathcal{A}$ as having an associated set of shapes - $X_{\mathcal{A}}$ (e.g. possible bird shapes), and an associated set of appearances - $Y_{\mathcal{A}}$ (e.g. possible bird appearances). With a similar interpretation for domain $\mathcal{B}$, we formalize the following problems:

\textbf{Intra-domain disentanglement:} where a method can generate images of the form $I = G(x, y, z, b)$, where $[x,y] \in (X_A \times Y_A)$ ($\times$ denotes Cartesian product). In other words, the task is to combine all possible shapes with the possible appearances \emph{within} a domain (e.g. $I_{AA}$ and $I_{BB}$ in Fig.\ref{fig:teaser}).\\ \textbf{Inter-domain disentanglement:} where everything remains the same as intra-domain disentanglement, except that $[x,y] \in (X_{AB} \times Y_{AB})$, where $X_{AB} = (X_A \cup X_B)$ and $Y_{AB} = (Y_A \cup Y_B)$. This is a more general version of the previous task, where we wish to combine all possible shapes with all possible appearances \emph{across} multiple domains (e.g. $I_{AB}$ in Fig.\ref{fig:teaser}).

We start with a base model which can perform unsupervised intra-domain disentanglement \citep{singh-cvpr2019}, the properties of which are summarized in Fig.\ref{fig:base}. Specifically, the base model generates an image using four latent vectors as input - $x$, $y$, $z$ and $b$ - each controlling object's shape, appearance, pose and background respectively. Furthermore, disentangling the foreground from background is handled by generating them separately, and combining them using a generated mask : $I = (m*I_f) + (1-m)*I_b$, where $I_f$, $I_b$ and $m$ are foreground, background and mask respectively. We now  explain how these properties could be used to extend the method’s ability from performing intra to inter-domain disentanglement.
% In the context of this work, we say that a generative model $G_{\mathcal{A}}$ is able to perform intra-domain disentanglement on domain $\mathcal{A}$ (e.g. birds), if and only if it is able to disentangle four factors of variations - pose, shape, appearance and background - while generating an image. This means that $G_{\mathcal{A}}$ takes four latent variables as input (one for each factor), and each variable controls the corresponding factor in the generated image. Fig.\ref{fig:base} summarizes these properties of $G_{\mathcal{A}}$; in each row, only one factor varies left to right, and all the other factors remain the same. Note that in order to accurately disentangle background from foreground (last row in Fig.\ref{fig:base}), the model needs to generate foreground in a separate layer, and will consequently generate the corresponding mask to stitch it with the background [issues in describing the concept of mask without describing FineGAN].  
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/base_model.pdf}
    \caption{Base model \citep{singh-cvpr2019} capable of performing intra-domain disentanglement for four factors of variation. Each of the four rows demonstrates the effect of changing one latent factor, which controls a single attribute in the image.}
    \label{fig:base}
\end{figure}

\subsection{Capturing shape independent representation of appearance}\label{sec:approx}
%The same base model which can combine shape and appearance effectively within a domain has trouble combining them across different ones. 
Although the base model can combine shape and appearance effectively within a single domain (Fig. \ref{fig:base} bottom left), it has trouble doing so across different ones. This is illustrated in Fig.\ref{fig:pos_neg}, where the behaviour of the same latent appearance vector is different when combined with a car's ($I$) versus a bird's shape ($I_{pos_{2}}$).

But what is it that makes the appearance of $I$ and $I_{pos_{2}}$ different? We observe that the car in $I$ is mostly red (body) and partly blue (windows), whereas the bird in $I_{pos_{2}}$ becomes completely blue. In other words, there is a discrepancy in the \emph{frequency} of certain visual concepts (RGB colors in this case) between $I$ and $I_{pos_{2}}$. We posit that reducing this discrepancy, i.e. making any two images with same latent appearance have similar frequency of visual concepts will lead to better appearance transfer across domains. To use this idea as part of an optimization process, however, we need to - (i) define the concepts whose frequency needs to be approximated, (ii) make the approximation process differentiable.  

It is difficult to pre-define the concepts which would be useful for an arbitrary pair of image domains; for example, a concept representing the leopard's texture might not be useful for shape/appearance disentanglement in \texttt{birds $\leftrightarrow$ cars}, but it would be in \texttt{animals $\leftrightarrow$ cars}. Hence, our idea is to learn these concepts in a data driven way. Specifically, we represent them using a set of learnable filters (Fig.\ref{fig:hist_rep}), each of which convolves over a generated image to give regions of high correlation. Focusing only on the object, we mask out the background using the foreground mask generated via the base model, and compute the channel-wise summation of the resulting response maps to get a $k$-dimensional representation. This representation approximates the frequency of visual concepts represented by the set of filters. 
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/hist_representation_new.pdf}
    \caption{Feature histogram approximation method. The base model, conditioned on multiple latent vectors, generates an image and it's foreground mask. Note that all the subsequent operations (e.g. convolution, element-wise multiplication) are differentiable, making the whole process usable for histogram equalization constraints.}
    \label{fig:hist_rep}
\end{figure}
How do we ensure that frequency is being approximated of some relevant feature? The information captured by the filter bank should be such that (i) same object in different pose/viewpoints has similar appearance representation, (ii) which in turn should be dissimilar than the representation of any other arbitrary object. Taking motivation from \citep{bachman-neurips2019, chen-arxiv2020}, we hence train the filter bank using a contrastive learning based setup. Specifically, we first construct a batch of $N$ generated images, where each image is of the form $I = G(x_1, y_1, z_1, b_1)$. We then construct another batch, where each image is of the form $I_{pos_{1}} = G(x_1, y_1, z_2, b_1)$, by only altering the noise ($z$) vector. Note that it is the property of our \emph{base model} through which we can assume that changing the noise vector will accurately retain the appearance of the foreground object, and would only change object pose/viewpoint (top-left row of Fig.\ref{fig:base}). This way, each of the corresponding images in $I$ and $I_{pos_{1}}$ will be positive samples. We get the frequency-based representation for all the $2N$ images, and calculate the $NT$-$Xent$ (Normalized temperature-scaled cross entropy loss) for each image in the batch :

\begin{equation}
\ell_{i}=-\log \frac{\exp \left(\operatorname{sim}\left(h_{i}, h_{j}\right) / \tau\right)}{\sum_{k=1}^{2 N} \mathbf{1}_{[k \neq i]} \exp \left(\operatorname{sim}\left(h_{i}, h_{k}\right) / \tau\right)}
\label{eq:filter}
\end{equation}
where $h_{i}$ represents the feature histogram of $i^{th}$ image, $j$ indexes the positive sample for $i$, and $\tau$ represents the temperature hyperparameter. We refer to the whole loss as $L_{filter} = \sum_{i=1}^{N} \ell_{i}$, and optimize it by only updating the weights of the filter bank. 

Given that we have a method to learn meaningful filters, we now use them for the core task our framework seeks to solve - combining latent appearance vector with arbitrary shapes such that the resulting appearance properties are similar. For this, we use an objective similar to $L_{filter}$ defined above, where we use the same $I = G(x_1, y_1, z_1, b_1)$. We construct the positive samples, however, differently - $I_{pos_{2}} = G(x_2, y_1, z_1, b_1)$ (latent shape representation $x$ is different than $I$). We refer to this loss as $L_{hist}$, and optimize $G$'s parameters, while keeping filter banks fixed. Intuitively, $L_{filter}$ is better optimized when filters capture characteristic low-level properties pertaining to a dataset (e.g. \emph{fur} texture pattern in \texttt{dogs $\leftrightarrow$ cars}). Consequently, optimization of $L_{hist}$ ensures that transferring a latent appearance (dog's fur) onto a different shape (car) better preserves those characteristic properties.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/contrastive_new.pdf}
    \caption{Positive/negative samples for different loss functions. Positive samples for $L_{filter}$ are the ones that we \emph{know} have similar appearance, whereas the positive samples for $L_{hist}$ are the ones that we \emph{wish} to have similar appearance. Negative samples remain the same for both $L_{filter}$ and $L_{hist}$.}
    \label{fig:pos_neg}
\end{figure}

% \begin{figure}
%     \centering
%     \subfloat[]{{\includegraphics[width=0.31\textwidth]{figs/diff_transfers.pdf}}}
%     \qquad
%     \subfloat[]{{\includegraphics[width=0.62\textwidth]{figs/contrastive_new.pdf}}}
%     \caption{(a) Transferring a car's appearance to a bird's body; (b) Positive/negative samples for different loss functions}
%     \label{fig:pos_neg}
% \end{figure}

\subsection{Base model}\label{sec:base_sec}
In principle, the framework described above should work with any base model that has the properties required to perform intra-domain disentanglement, as decsribed in Sec. \ref{sec:formulation}. To the best of our knowledge, however, FineGAN \citep{singh-cvpr2019} is the only method meeting those requirements in an unsupervised manner. It takes in four latent variables as input - a continuous noise vector $z \sim \mathcal{N}(0,1)$, and one-hot vectors $x \sim \text{Cat}(K = N_x,p = 1/N_x)$, $y \sim \text{Cat}(K = N_y,p = 1/N_y)$ and $b \sim \text{Cat}(K = N_b,p = 1/N_b)$, where $N_x$, $N_y$ and $N_b$ represent the number of distinct shapes, appearances and background to be discovered. FineGAN takes in these sampled codes, and generates an image in a stagewise manner, where background and foreground are generated separately and stitched together using a generated foreground mask. To learn the desired disentanglement, FineGAN makes the assumption that $N_x < N_y$, i.e. varieties in shapes is less than different appearances of objects. This is especially true in the context of fine-grained image datasets, for e.g. all ducks having different appearances have the same overall shape. During training, this \emph{hierarchy constraint} is imposed in the process of constructing latent vectors, where a set of appearance vectors ($y$) will always be paired with a particular shape vector ($x$). This ensures that, during training, the shape vector representing the duck's shape does not get paired up with the appearance vector for sparrow's texture to create some unnatural combination (which could be used by a discriminator to easily classify the image as fake). Two types of loss functions are used - $L_{abv}$, i.e. the adversarial losses \citep{goodfellow-nips2014} to enforce realism on the background image and the final image ($I$), and mutual information loss $L_{info}$ \citep{chen-nips16} between (i) $x$ and foreground shape, (ii) $y$ and foreground appearance, to help the latent vectors get control over the respective factors. We denote the loss functions used by the base model (FineGAN in this case) as $L_{base}$.

So, the overall loss function used by our framework becomes:
\begin{equation}
\mathcal{L} = L_{base} + L_{hist} + L_{filter}    
\end{equation}
where $L_{base}$ constrains the model to have the properties needed for intra-domain disentanglement, and the combination of $L_{filter}$ and $L_{hist}$ helps extent the abilities to learn inter-domain disentanglement of factors.  
% If we wish for any two generated images $I_1$ and $I_2$ with arbitrary shapes to have the same appearance details, the idea of feature histogram equalization of $I_1$ and $I_2$ seems promising. But to ensure that background details are not considered as part of histogram equalization, our generative model needs to be able to disentangle background from foreground while generating the complete image. 
% To this end, we build upon the recent work of FineGAN [refer], which is an unsupervised generative model that can (i) disentangle the background from foreground; (ii) perform intra-domain disentanglement between shape and appearance, as described in Fig.\ref{fig:teaser}. In the next section, we briefly describe the core components of FineGAN, and give a high-level overview of it's strengths and weaknesses in terms of qualitative results. We then introduce our framework which can blend in with FineGAN's model to enable inter-domain disentanglement.

% \subsection{FineGAN}
% FineGAN proposed a generative model which can take in four latent variables $z$, $b$, $p$ and $c$
% The premise of FineGAN is centered around a property that many \emph{fine-grained} image datasets tend to follow: if the visual differences between images belonging to object category $c_1$ and $c_2$ are indeed fine-grained (e.g. only the spots on the tail of a bird are differently colored for $c_2$ than $c_1$, but the rest of the body is same as $c_1$), then this could be understood as similarity in one of the latent factors, and difference in some other. So, in a dataset of $n$ fine-grained categories, a hierarchy of latent factors could be imagined, where a subset of $n_1$ fine-grained categories would have the same parent latent factor $p_1$.

% The core idea of the work then becomes to disentangle the factors present at different levels of this potential hierarchy. Since there is no human-level annotation for this latent hierarchy, FineGAN assumes one based on some heuristics (e..g # of parent nodes < # of child nodes; some children will share the same parent nodes). This hierarchy is enforced through the latent variables  


==> introductionv1.tex <==


\section{Introduction}
Combining properties from multiple image distributions to create novel visual concepts is an incredible ability that humans possess. An example of this is discussed in \cite{lake-science2015}, about our ability to parse different object parts (e.g. wheels of a car, handle of a lawn mower) and combine them to conceptualize novel object categories (a scooter). Fig.\ref{fig:teaser} illustrates this ability through a different angle; it is easy for us humans to imagine how the brown car would look if it's appearance were borrowed from the blue/red bird, and vice versa. To model a similar ability in machines, a precise disentanglement of shape and appearance features, and the ability to combine them across different domains should be present; and in this work, we seek to develop a framework to do that.    

Disentangling the factors of variation in visual data has received significant attention \citep{chen-nips16, higgins-iclr2017, denton-nips17, singh-cvpr2019}, in particular with advances in generative models \citep{zhang-tpami2018, karras-cvpr19}. The premise behind learning disentangled representations is that an image could be thought of as a function of, say two independent latent factors, such that each controls only one human interpretable property (e.g. shape vs. appearance). Existence of such representations enables combining latent factors from different source images to create new one having properties of both the source images. Prior work has explored a part of this idea, where the space of latent factors being combined is constrained to be within one domain (e.g. combining sparrow's appearance with duck's shape; $I_{AA}$ in Fig.~\ref{fig:teaser}), a scenario which we refer to as \emph{intra-domain} disentanglement of latent factors. In this work, we wish to generalize this idea by developing a framework which can combine latent factors from different domains (e.g. appearance/shape from a bird/car respectively) to create a new breed of images which does not exist in either domains ($I_{AB}$ in Fig.~\ref{fig:teaser}). 
Furthermore, this generalization also offers an opportunity to test any entanglement which might have gone unnoticed when only dealing with intra-domain disentanglement. In other words, if a method can learn disentangled latent representations within a domain effectively (e.g. can transfer the appearance of a sparrow to a duck's body), but performs poorly in terms of learning similar representations in the presence of multiple domains (e.g. cannot transfer the appearance of a yellow sparrow to a car), that in essence indicates some form of entanglement of the appearance feature with the \emph{bird-like} shape. 

Specifically, we focus on two factors: shape and appearance details of an object, and present a framework that can combine these two factors from different domains to generate hybrid images, e.g. $I_{AB}$ in Fig.\ref{fig:teaser}, where $AB$ represents shape and appearance being taken from domains $A$ and $B$ respectively. 

Inter-domain transfer is difficult (ill posed) since correspondences are unclear, but one sensible heuristic is the one that humans use to evaluate the effectiveness of appearance transfer. Looking back at Fig.\ref{fig:teaser}, the goal is to transfer the appearance of the red/blue bird to the brown car. Even without any object part correspondence between a bird and a car's shape (i.e., should a bird's wing color go to the car's door or roof or some other part?), we can deduce that $I_{AB}$ represents a successful transfer. This is because the \emph{frequency of visual features} over the bird's body is very similar to the one over the car's body, where visual features in this case represents a combination of red and blue color, but could represent something more complex (e.g. some texture pattern).
To capture this intuition, we propose a simple framework which can approximate a histogram of visual features (e.g. texture, color, some combination of both) of an object in a differentiable way using the responses of a filter bank, and can consequently constrain the approximated histograms of any two images (having the same latent appearance vector but different shape) to be the same. Furthermore, to enable the construction of histogram in a data-driven way (as opposed to a hard-coded feature), we present a contrastive learning setup \cite{hadsell-cvpr06, chen-arxiv2020} to train our filter bank to better align with the dataset under consideration.
In principle, our overall framework could be used in conjunction with any method capable of performing intra-domain disentanglement, and helps extend the method's ability to better perform in terms of inter-domain disentanglement. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/teaser_new.pdf}
    \caption{Each domain could be thought of as having a set of potential shapes ($X_A/X_B$) and appearance ($Y_A/Y_B$). Ability to generate images of the form $I_{AA}/I_{BB}$ requires the system to learn intra-domain disentanglement \citep{singh-cvpr2019} of latent factors, whereas the ability to generate images of the form $I_{AB}$ (appearance/shape from domain A/B respectively) requires inter-domain disentanglement of factors, which is the goal of this work.}
    \label{fig:teaser}
\end{figure}
To the best of our knowledge, our work is the first to attempt combining factors from different data distributions to generate abstract visual concepts (e.g. tiger in dog's texture, car in bird's color). We demonstrate the applicability of this framework on a variety of multi-modal datasets, and demonstrate better performance, qualitatively and quantitatively, over baselines. 
Overall, our hope with this work is to pave the way for a new breed of algorithms which can extract information from multiple data distributions to create new visual concepts.

==> introductionv2_orig.tex <==


\section{Introduction}
Combining properties from multiple image distributions to create novel visual concepts is an incredible ability that humans possess. An example of this is discussed in \citet{lake-science2015}, about our ability to parse different object parts (e.g. wheels of a car, handle of a lawn mower) and combine them to conceptualize novel object categories (a scooter). Fig.\ref{fig:teaser} illustrates this ability through a different angle; it is easy for us humans to imagine how the brown car would look if it's appearance were borrowed from the blue/red bird, and vice versa. To model a similar ability in machines, a precise disentanglement of shape and appearance features, and the ability to combine them across different domains should be present; and in this work, we seek to develop a framework to do that.    

Disentangling the factors of variation in visual data has received significant attention \citep{chen-nips16, higgins-iclr2017, denton-nips17, singh-cvpr2019}, in particular with advances in generative models \citep{zhang-tpami2018, karras-cvpr19, radford-iclr2016, brock-iclr2019}. The premise behind learning disentangled representations is that an image could be thought of as a function of, say two independent latent factors, such that each controls only one human interpretable property (e.g. shape vs. appearance). Existence of such representations enables combining latent factors from two different source images to create new one, having properties of both. Prior work \citep{singh-cvpr2019, li-cvpr2020} has explored a part of this idea, where the space of latent factors being combined is limited to one domain (e.g. combining sparrow's appearance with duck's shape; $I_{AA}$ in Fig.~\ref{fig:teaser}), a scenario which we refer to as \emph{intra-domain} disentanglement of latent factors. This work, focusing on shape and appearance as factors, generalizes this idea by combining latent factors from different domains (e.g. appearance from birds, shape from cars) to create a new breed of images which does not exist in either domains ($I_{AB}$ in Fig.~\ref{fig:teaser}). \kr{should we mention briefly why prior work can't do inter-domain?}

Even without a ground-truth distribution for this new breed, there are heuristics we can use to assess how well these factors combine across domains. For example, the foreground appearance of $I_2$ and $I_{AB}$ is somewhat similar, because the frequency of certain low-level features (e.g. RGB colors) remains consistent in both of them. Our work formulates this idea as part of a training process, where any two images having the same latent appearance ($I_2$/$I_{AB}$) are constrained to have similar frequency of those low-level features. These features in turn are \emph{learnt} (as opposed to being hard-coded), using a contrastive learning setup \citep{hadsell-cvpr06, chen-arxiv2020}, to better approximate the low-level statistics of the dataset. The net effect is an accurate transfer of appearance, where important details about it remain consistent across domains. 

\begin{figure}[t]
    \begin{minipage}[c]{0.72\textwidth}
    \includegraphics[width=1\textwidth]{figs/teaser_compressed.pdf}
    \end{minipage}\hfill
    \begin{minipage}[c]{0.28\textwidth}
    \caption{Each domain could be represented as a set of shapes ($X_{A/B}$) and appearance ($Y_{A/B}$). Ability to generate images of the form $I_{AA/BB}$ requires the system to learn intra-domain disentanglement \citep{singh-cvpr2019} of latent factors, whereas the ability to generate images of the form $I_{AB}$ (appearance/shape from domain A/B respectively) requires inter-domain disentanglement of factors, which is the goal of this work.}
    \label{fig:teaser}
    \end{minipage}
\end{figure}
To the best of our knowledge, our work is the first to attempt combining factors from different data distributions to generate abstract visual concepts (e.g. tiger in dog's texture). This opens up new avenues to creating art: (i) a customer could visualize how the sofas would look with an animal print, (ii) a fashion/car designer could create a new space of designs using appearance from arbitrary objects. In this work, we show the applicability of our method on a variety of multi-modal datasets, and demonstrate effectiveness qualitatively, quantitatively, and through user studies. Finally, we believe that the task introduced in this work offers better scrutiny of the quality of disentanglement learnt by a method: if it succeeds in doing so within a domain but not in the presence of multiple ones, that in essence indicates some form of entanglement of a factor with the domain's properties. 

==> relatedv1.tex <==
\section{Related work}

\paragraph{Disentangling shape and appearance.} In recent years, there has been a lot of work in disentangling object appearance from its shape (\cite{peng-iccv2017,balakrishnan-cvpr2018,ma-cvpr2018,esser-cvpr2018,li-ijcai2018,shu-eccv2018}). Many of these are supervised \citep{peng-iccv2017,balakrishnan-cvpr2018,ma-cvpr2018} and rely on key-points and masks. Some approaches \citep{li-ijcai2018,shu-eccv2018} try to overcome this limitation and learn to disentangle shape and appearance in unsupervised way. Works like FineGAN \citep{singh-cvpr2019} and MixNMatch \citep{li-cvpr2020} went beyond just disentangling two factors and disentangled background, pose, shape, and appearance. However, all these approaches are restricted to a single dataset with a single high-level class and does not generalizes well for multiple datasets having variety of object categories. The naive approach of just combining multiple datasets to train the disentanglement model fails as it learns shapes specific to a dataset. As a result, appearance does not transfer well across the shapes corresponding to different datasets. Our approach tries to overcome this issue by enforcing explicit constraints to enable appearance transfer across the shapes corresponding to different datasets.

\paragraph{Style transfer.} In the past few years, networks \citep{gatys-arxiv2015,johnson-eccv2016,ulyanov-icml2016} have been proposed to generate a new image by taking content from one image and style from another image. These approaches try to transfer style from an image by matching global color/texture image statistics of a pre-trained model and cannot have style correspondence at the local part level when part correspondence exists between two images. CycleGAN and its variants \citep{zhu-cvpr2017,kim-icml17} proposed a more general approach to transfer style between two image domains rather than two specific images and can transfer style at a part level when the part correspondence exists between the classes of two domains. However, they can generally transfer styles between the two domains only if their classes have very similar shapes and global structures. In contrast to these methods, our approach can transfer color/texture details between two domains having classes with very different shapes and can also do it at the local part level if the correspondence exists between the classes of two domains (e.g. cats and dogs). Apart from that, unlike previous methods our approach can only transfer color/texture among the foreground region without affecting the background.

\paragraph{Domain adaptation and cross dataset disentanglement.} There has been a lot of GANs based domain adaptation work \citep{ganin-jmlr2016,hoffman-arxiv2016,lee-eccv2018} to improve various recognition tasks like image classification and segmentation. Most of these approaches try to learn domain agnostic feature representation, so that they can fool discriminator which is trying to identify the domain of the feature. However, to the best of our knowledge, we do not know any domain adaption work which tries to learn better disentanglement between two domains which is the goal of our work. Recently, there have been some promising works \citep{gonzalez-nips2018,sendik-arxiv2020} on the cross dataset disentanglement. However, \cite{gonzalez-nips2018} make the assumption that there should be some shape similarity between two domains whereas \cite{sendik-arxiv2020} requires similar color/textures to be present in the two domains for the disentanglement to be learned. Our approach does not have these constraints and can work for the domains with drastically different shapes and no color/texture similarity.

==> resultsv1.tex <==
\section{Results}\label{sec:results}
We now compare the proposed framework against several baselines, and study how they fare in terms of combining shape and appearance from different domains. We first define the multi-domain datasets and baselines used for evaluation. We then define the metrics used to quantify the accuracy of color and texture preservation while transferring appearance to an arbitrary shape. We then present and analyze the qualitative results, demonstrating the effectiveness of our approach.

\subsection{Datasets and baselines}
We use three single domain datasets: \textbf{(i) CUB} consists of 11,788 bird images belonging to 200 fine-grained categories. \textbf{(ii) Stanford Dogs} consists of 12,000 training images belonging to 120 dog categories. \textbf{(iii) Stanford Cars} consists of 8,144 images belonging to 196 categories of cars. Using these, we construct three multi-domain settings : \textbf{(i) birds $\leftrightarrow$ cars}, \textbf{(ii) cars $\leftrightarrow$ dogs}, \textbf{(iii) dogs $\leftrightarrow$ birds}, consisting of a total of 396, 316 and 320 object categories respectively. Apart from these, we also evaluate on a dataset of animal faces (\cite{liu-iccv19}), consisting of a total of 117,484 images belonging to 149 carnivorous categories, where each category could be interpreted as a different domain. This forms our fourth multi-domain setting, \textbf{(iv) animals $\leftrightarrow$ animals}.  

We compare against the following baselines on the mentioned datasets: \textbf{(i) FineGAN \citep{singh-cvpr2019}} - This is the base model described in Sec.\ref{sec:base_sec}, where both $L_{adv}$ and $L_{info}$ are used on images of the form $G(z, x, y, b)$, with $x$ and $y$ constrained in a hierarchical way. \textbf{(ii) Relaxed FineGAN} - We design this baseline based on FineGAN, where in each iteration we first have $L_{base}$ (all the $L_{adv}$ and $L_{info}$ based losses) applied on images of the form $G(z, x, y, b)$ where $x$. In the next iteration, however, we release the \emph{hierarchy constraint} (refer to Sec. \ref{sec:base_sec}) and optimize only $L_{info}$.\textbf{(iii) AdaIn \citep{huang-iccv2017}} - This work presented a method to transfer \emph{style} of an image to an arbitrary content image. Although style vs content disentanglement is somewhat related, we show why style-transfer methods will fail to perform the kind of disentanglement we're studying in this work. \textbf{(iv) Ours} w/o $L_{filter}$ - This is our approach when we simply use a randomly initialized filter bank to approximate the feature histogram, and don't using $L_{filter}$ to tune it. \textbf{(v) Ours} - This is our final approach.
For all the baselines, we use $N_y$ (no. of discrete appearances in the dataset) as the total number of categories, and $N_x$ (no. of discrete shapes) as $N_y/10$, i.e. we assume that a set of 10 object categories share a common shape. For \textbf{birds $\leftrightarrow$ dogs} setting, for example, this would make $N_x = 32$ and $N_y = 320$. Note that we borrow this assumption from FineGAN, as that is what we're using as the base model.  For all the other training details (e.g. hyperparameters), please refer to the supplementary.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/birds_cars_res.pdf}
    \caption{Results on \textbf{birds $\leftrightarrow$ cars}. The only difference between the 'Output' and 'Shape' image is of the latent appearance vector, which is borrowed from the 'Appearance' image. Our method results in a much more accurate transfer of appearance from one shape to another (e.g. row 1).}
    \label{fig:birds_cars}
\end{figure}
\subsection{Analysis}
We now discuss how the aforementioned baselines fare in terms of disentangling appearance and shape of the objects during generation. More specifically, given images $I_1 = G(x_1, y_1, b_1, z_1)$ and $I_2 = G(x_2, y_2, b_2, z_2)$ from two different domains, we study how well the shape and appearance of $I_1$ and $I_2$ are preserved in $I_3 = G(x_1, y_2, b_1, z_1)$. 
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/dogs_cars_res.pdf}
    \caption{Results on \textbf{cars $\leftrightarrow$ dogs}. Similar relations are followed between the 'Appearance', 'Shape' and 'Output' images as described in Fig.~\ref{fig:birds_cars}. Our method not only results in accurate color transfer, but also in transfer of other low level details, e.g. golden fur in row four.}
    \label{fig:dogs_cars}
\end{figure}
\subsubsection{Qualitative analysis}
\paragraph{Issues with the baselines:} Figures \ref{fig:birds_cars}, \ref{fig:dogs_cars} and \ref{fig:animals} summarize the results over multiple datasets. 
%The results for AdaIn \cite{huang-iccv2017} are generated by treating the appearance and shape images as style and content images (according to the style-transfer literature) respectively. 
We observe that both FineGAN and AdaIn have trouble transferring appearance from one object to another one. As for AdaIn, it can only extract \emph{style} (texture based features), which might not capture the holistic appearance of an object (e.g. Fig.~\ref{fig:animals} rows 1, 3 and 4: the desired appearance is not transferred). Furthermore, AdaIn (or any style-transfer algorithm) can only transfer style of the complete source image to \emph{all} the spatial locations in the target image, which results in unnatural artifacts (e.g. Fig. \ref{fig:birds_cars} row 1, transferring the appearance of the red car to a bird results in reddish patches in the background of target image). FineGAN, on the other hand, sometimes results in a highly inaccurate appearance transfer (e.g. Fig. \ref{fig:birds_cars} row 1: only car's window's color gets transferred to the bird).  There are other cases which demonstrate transfer of only the \emph{rough color} to the target object shape, but not the signature appearance details: e.g. 
%rough transfer of yellow color in row 3 of Fig.~\ref{fig:birds_cars}, 
transfer of brown color from dog's fur to the car in row 4 of Fig.~\ref{fig:dogs_cars}, but not the \emph{fur texture} of the dog. 

Our approach, on the other hand, results in a more \emph{holistic} transfer of appearance. It maintains the relative frequencies of visual features during transfer, e.g. Fig.~\ref{fig:birds_cars} row 2 demonstrates the transfer of both the blue and red components to the car. Furthermore, ours method can also capture and transfer the minute details of the appearance of an object. For example, in Fig.~\ref{fig:dogs_cars} row 4, we see that the dog has \emph{golden} \emph{fur}, and transferring that appearance it results in a car with \emph{golden} \emph{fur} stuck over it's body. Row 3 in the same figure further shows the transfer of an irregular-shaped appearance from dog to a car, which is not the case with FineGAN, which only transfers the less dominant color from dog to car. Note that inputs to our/FineGAN's method are latent vectors spanning multiple domains, whereas AdaIn is an image conditional algorithm taking appearance/shape (analogous to style/content) images as input. We use our algorithm's source appearance/shape images as the style/content input respectively.   

\paragraph{Resistivity issue:} In Fig. \ref{fig:animals}, we see that FineGAN shows a \emph{resistance} towards changing the appearance of an animal; e.g. in row 4, the leopard  in the target image only borrows a blackish color tone, and most of the signature leopard appearance remains as it is. In contrast, our method is able to comprehensively change the appearance of an animal; e.g. in the same row, leopard can shed its appearance and borrow everything from the tricolored dog, while also preserving any potential correspondence (the resulting animal retains the brown patch above the eye). We study the resistivity property in more detail: for each latent shape vector $x_i$, we construct a list of images ($L$) by combining it with all possible latent appearance vectors, keeping the latent noise ($z$ capturing pose) and background vectors the same, i.e.  $L$ = $\{G(x_i, y_j, z_i, b_i)\}$ $\vee y_j \in$ \textbf{animals $\leftrightarrow$ animals}. We then stack the images in $L$, compute standard deviation across channels separately, and then average to generate a heatmap image. We repeat this process for all the latent shape vectors, and plot the histogram of standard deviation values. 
Fig.~\ref{fig:animals_std} illustrates this process, and compares the heatmap images generated using our approach vs FineGAN. This helps us visualize the \emph{resistance} property, as the heatmap and histogram through FineGAN indicates much lower standard deviation of pixel differences compared to our approach, implying more diversity of visual appearance attainable using our method. 


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/animals_res.pdf}
    \caption{Results on \textbf{animals $\leftrightarrow$ animals}. Similar relations are followed between the 'Appearance', 'Shape' and 'Output' images as described in Fig.~\ref{fig:birds_cars}. Not only our method results in an accurate transfer of appearance from one animal to another, it does so by preserving the correspondence (e.g. brown patch above the eye of tiger in row four).}
    \label{fig:animals}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\textwidth]{figs/std_hist_test2.pdf}
    \caption{Analysis of the resistance of a model to alter the appearance. Generations using FineGAN don't fully relinquish the appearance, resulting in a low standard deviation for pixel changes across the spatial locations compared to our approach.}
    \label{fig:animals_std}
\end{figure}

\subsubsection{Quantifying appearance transfer}
We measure similarity in the foregrounds of two objects using - \textbf{(i) Color histogram:} which can be used to compare the relative frequencies of RGB values in two different objects; \textbf{(ii) Texton histogram:} \citep{leung-ijcv2001, varma-cvpr2003} which is used to compute the frequency of small texture patches belonging to a pre-defined codebook. We first define the process of obtaining the image and texture based cluster centers (codebook), and then explain the process of constructing and comparing the respective histogram representations of two images.

We sample 50,000 pixel (RGB) values randomly from the images belonging to a multi-domain dataset (e.g. \textbf{birds $\leftrightarrow$ cars}), and perform \emph{k-means} clustering with $k = 50$ to get the color centers. To compute the texture centers, the images in the dataset are first convolved with a MR8 \citep{leung-ijcv2001} filter bank, consisting of 38 filters and 8 responses capturing edge, bar and rotationally symmetric features. After this step, the process is similar to computing the color histograms: we sample 50,000 points from the images, each point being 8-dimensional, and cluster them into 50 centers representing the texton codebook. We repeat this process of computing the color and texture clusters for each multi-domain setting separately. For each latent appearance vector $y_i$, we generate a source image $I_s = G(x_i, y_i, b_i, z_i)$ and a target image $I_t = G(x_j, y_i, b_i, z_i)$ such that $x_i, y_i$ belong to one domain and $x_j$ to another (e.g. $x_i/x_j$ represents bird/car shape). We then use a semantic segmentation network (DeepLabv3 \citep{chen-arxiv2017}) pre-trained on PASCAL VOC 2012 \citep{pascal-voc-2012} to extract foreground pixels, and compute and compare color/texture based histograms between source and target images (more details in supplementary). Note that $I_t$ is likely to represent some visual concepts which were never seen by the segmentation network pre-trained on real data (e.g. car with dog's fur in Fig.~\ref{fig:dogs_cars}), which could result in unreliable segmentations from the network. We circumvent that by generating an intermediate image $G(x_j, y_j, b_j, z_i)$ such that both the appearance/shape factors belong to the same target domain. We then run the pre-trained segmentation network on this image, and use the  predicted foreground locations for $I_t$ (which has the same shape factor, $x_j$).

Table~\ref{tab:ct} summarizes the effectiveness of different methods in preserving the color/texture information when transferred to an object of different domain. We use $\chi^2$-distance to compute distance between the color/texture based histograms of source ($I_s$) and target ($I_t$) images. When considering color histogram similarity, we see that AdaIn performs poorly even when compared with FineGAN, which is evident especially through figures \ref{fig:birds_cars}, \ref{fig:dogs_cars}, where it has trouble altering the appearance of shape (or content) image. Note that 'Ours - $L_{filter}$' itself is a decent baseline, which simply uses random orthonormal initialization of the filter bank to minimize $L_{hist}$. Our final approach, which fine-tunes the filters, achieves the best overall performance in terms of retaining the RGB and texture information (within the capacity of MR8 filters). 






% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/std_img.pdf}
%     \caption{Standard deviation image}
%     \label{fig:dogs_cars}
% \end{figure}



\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{c|cc|cc|cc|cc}
%\hline
                & \multicolumn{2}{c|}{\textbf{birds $\leftrightarrow$ cars}} & \multicolumn{2}{c|}{\textbf{cars $\leftrightarrow$ dogs}} & \multicolumn{2}{c|}{\textbf{dogs $\leftrightarrow$ birds}} & \multicolumn{2}{c}{\textbf{animals $\leftrightarrow$ animals}} \\ \hline
                & \textbf{color}         & \textbf{texture}         & \textbf{color}         & \textbf{texture}        & \textbf{color}         & \textbf{texture}         & \textbf{color}            & \textbf{texture}           \\ 
FineGAN \citep{singh-cvpr2019}        & 0.4295               & 0.4234                 &      0.3856         &     0.4006           &       0.2862        &    0.3442             &       0.1914           &   0.2322                \\ 
Relaxed FineGAN & 0.3121               &  0.4005               &      0.3451         &      0.3912          &       0.2433        &         0.3287        &         0.1214         &        0.1834           \\ 
AdaIn   \citep{huang-iccv2017}       &   0.5619           &       0.4476          &      0.5113         &        0.3956        &      0.6265         &      0.3512           &          0.2447       &        0.1801           \\  \hline
Ours w/o $L_{filter}$  & 0.2842               &     0.3341            &     0.2289          &   0.2754             &      0.2228         &        0.2744         &    0.0721              &         0.0815          \\ 
Ours            &   \textbf{0.2484}             &   \textbf{0.3057}              &      \textbf{0.2069}         &  \textbf{0.2535}              &       \textbf{0.2009}        &        \textbf{0.2573}         &       \textbf{0.0462}           &     \textbf{0.0695}              \\ 

\end{tabular}

\vspace{2pt}
\caption{$\chi^2$-distance between the color/texture based histograms of source and target images. The bottom two methods use the idea of feature based histogram equalization. Enforcing similarity of the frequency of appropriate visual features (using $l_{filter}$ + $L_{hist}$) helps the model better retain hard-coded appearance properties (color/texture) as well.}
\label{tab:ct}
\end{table}


\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{c|c|c}
                & Ours vs AdaIn & Ours vs FineGAN \\
                \hline
\textbf{birds $\leftrightarrow$ cars}      & 77.82         & 70.12           \\
\textbf{cars $\leftrightarrow$ dogs}       & 75.32         & 63.28           \\
\textbf{dogs $\leftrightarrow$ birds}      & 79.95         & 73.26           \\
\textbf{animals $\leftrightarrow$ animals} & 82.51         & 76.21           \\ \hline
Average                & 78.90 $\pm$ 2.65  & 70.72 $\pm$ 4.81   
\end{tabular}
\caption{AMT results}
\end{table}


